Locality-Sensitive Orderings and Applications to Reliable Spanners

Chan, Har-Peled, and Jones [2020] recently developed locality-sensitive ordering (LSO), a new tool that allows one to reduce problems in the Euclidean space $\mathbb{R}^d$ to the $1$-dimensional line. They used LSO's to solve a host of problems. Later, Buchin, Har-Peled, and Ol{\'{a}}h [2019,2020] used the LSO of Chan {\em et al. } to construct very sparse \emph{reliable spanners} for the Euclidean space. A highly desirable feature of a reliable spanner is its ability to withstand a massive failure: the network remains functioning even if 90\% of the nodes fail. In a follow-up work, Har-Peled, Mendel, and Ol{\'{a}}h [2021] constructed reliable spanners for general and topologically structured metrics. Their construction used a different approach, and is based on sparse covers. In this paper, we develop the theory of LSO's in non-Euclidean metrics by introducing new types of LSO's suitable for general and topologically structured metrics. We then construct such LSO's, as well as constructing considerably improved LSO's for doubling metrics. Afterwards, we use our new LSO's to construct reliable spanners with improved stretch and sparsity parameters. Most prominently, we construct $\tilde{O}(n)$-size reliable spanners for trees and planar graphs with the optimal stretch of $2$. Along the way to the construction of LSO's and reliable spanners, we introduce and construct ultrametric covers, and construct $2$-hop reliable spanners for the line.

==> LSO-doubling.tex <==
\section{LSO for Doubling Metrics}\label{sec:LSOdoubling}
We will use the following lemma:

\begin{lemma}\label{lm:filtser-cover}  Consider a metric space $\left(X,d_{X}\right)$ of	doubling dimension $d$, and parameters $\Delta$, then for every	$t=\Omega(1)$, there is a set of $O(2^{\frac{d}{t}}\cdot d\cdot\log t)$	partitions, such that every pair of points at distance at most $\Delta$ belongs to some cluster in some partition, and every cluster in every partition has diameter at most $O(t)\cdot\Delta$.
\end{lemma}

This section is devoted to the proof of \Cref{thm:DoublingLSO}, we restate it for convinience.
\DoublingLSO*
%\begin{restatable}[LSO For Doubling Metrics]{theorem}{DoublingLSO}
%	\label{thm:DoublingLSO}
%	Every metric space $(X,d_{X})$ of doubling dimension $d$, admits an $\left(O_{d}(\epsilon^{-d}\log\frac{1}{\epsilon}),\epsilon\right)$-LSO.
%\end{restatable}
\atodoin{I changed the original number of ordering from $O_{d}(\epsilon^{-d}\log\frac{1}{\epsilon})$ to $O(\epsilon)^{-d}\log\frac{1}{\epsilon}$ . Perhaps better to change also in \Cref{thm:CHJ20EuclideanLSO}}
\begin{proof}
	We assume that the minimum distance is $1$. Consider $O(\log(1/\epsilon))$ scales:
	
	\begin{equation}
	\begin{split}
	S_{1}&=\{[1,2),[1/\epsilon,2/\epsilon),...,[1/\epsilon^{i},2/\epsilon^{i}),\ldots,\}\\
	S_{2}&=\{[2,4),[2/\epsilon,4/\epsilon),...,[2/\epsilon^{i},4/\epsilon^{i}),\ldots,\}\\
	&\ldots\\
	S_{O(\log1/\epsilon)} &=\{[\frac{1}{2\epsilon},\frac{1}{\epsilon}),[\frac{1}{2\epsilon^{2}},\frac{1}{\epsilon^{2}}),...,[\frac{1}{2\epsilon^{i+1}},\frac{1}{\epsilon^{i+1}}),\ldots,\}
	\end{split}
	\end{equation}

	For each scale $S_{j}$, define a set of edges $E_{j}=\{(x,y):d_{X}(x,y)\in[2^{j-1}/\epsilon^{i},2^{j}/\epsilon^{i}\mbox{ for some }i\}$. We then construct a locality sensitive ordering $\Sigma_{j}$ for
	each $E_{j}$ in the following sense: for each $(x,y)\in E_{j}$,
	there is an ordering $\sigma\in\Sigma_{j}$ such that $x$ and $y$
	are \emph{properly order in $\sigma$: }$x\prec_{\sigma}y$ and $\forall z\in\sigma(x,y):\min(||x,z||,||y,z||)\leq O(\epsilon)||x,y||$.
	($\sigma(x,y)$ is the set of all points between $x$ and $y$ in
	$\sigma$.)
	
	
	Let $L_{i}=$$2^{j}/\epsilon^{i}$ to be an upper bound on edges at
	level $i$ of $E_{j}.$ For each level $i$ of scale $S_{j}$, let
	$\mathcal{P}_{i}$ be a set of $O(2^{d})$ partitions of X such that
	for every partition $\Pi\in\mathcal{P}_{i}$, every cluster $C\in\Pi$
	has diameter at most $10L_{i}$.  We say an edge $(x,y)\in E_{j}$ \emph{covered by partition $\Pi\in\mathcal{P}_{i}$} if there exists $C\in\Pi$
	such that $B(x,4L_{i-1})\cup B(y,4L_{i-1})\subseteq C$.
	\begin{lemma}\label{lm:cover-edge}
		For every edge $(x,y)$ at level $i$ of $E_{j}$, there exists $\Pi\in\mathcal{P}_{i}$ that covers $(x,y)$.
	\end{lemma}
	
	\begin{proof} Follows from the fact that the set partition $\mathcal{P}_{i}$ is a sparse cover.
	\end{proof}

	Let $p=2^{O(d)}$ be the upper bound on the numer of partitions
	in $\mathcal{P}_{i}$. We assume that each $\mathcal{P}_{i}$ has
	\emph{exactly $p$ }partitions by duplicating if neccessary. We then
	fixed an (arbitrary) linear order on partitions in $\mathcal{P}_{i}$.
	We then construct $p$ \emph{hierarchies of partitions} $\mathcal{H}_{1,}\mathcal{H}_{2},\ldots,\mathcal{H}_{p}$ as follows: for $k$-th hierachy $\mathcal{H}_{k}$, we take $k$-th partition of $\mathcal{P}_{i}$ to be the level $i$ of $\mathcal{H}_{k}$. Note here that clusters at different levels may not be nested, i.e, points in a cluster at level $i-1$ may belong to two different clusters at level $i$.
	
	
	We say that edge $(x,y)\in E_{j}$ at level $i$ \emph{is covered} by hierarchy 	$\mathcal{H}$$_{k}$ if $(x,y)$ is covered by the partition at level	$i$ of $\mathcal{H}_{k}$. 
	
	\begin{lemma}\label{lm:cover-hierarchy}
		For every edge $(x,y)$ at level $i$ of $E_{j}$, there exists a hierachy
		$\mathcal{H}_{k}$ that covers $(x,y)$.
	\end{lemma}
	\begin{proof} Follow directly from Lemma~\ref{lm:filtser-cover} and Lemma~\ref{lm:cover-edge}.
	\end{proof}

 We construct a tree $T$ from $\mathcal{H}_k$ as follows:
 	\begin{enumerate}
 		\item Level $0$ are singletons, all are active.
 		\item For level-$i$, let $\Pi$ be the corresponding parition. We do the following.
 			\begin{enumerate}
 				\item For every cluster $C \in \Pi$ that has at least two active  points  $\{x_1,\ldots, x_c\}$. Elect $x_1$ to be the parent of $x_2,\ldots, x_{c}$, and mark all $\{x_2,\ldots, x_{c}\}$ to be \emph{inactive}. 
 			\end{enumerate}
 	\end{enumerate}
 
 A technical twist is that we need to guarantee that elected points at the same level $i$ of $T$ must be far from each other, say distance $L_i/2$ from each other; so that they "behave" like a net. There is a couple of ways to enforce this, for example, by choosing a net from these elected points and ``merge'' subtrees of points that are too close. We omit the dettails here, and for simplicity, just assme that elected points at level $i$ have distances $\Omega(L_i)$ from each other. This implies that:
 
\begin{lemma}\label{lm:children} For every node $t\in T$, it has at most $O(\epsilon^{-d})$ children.
\end{lemma} 

The following lemma is standard:

\begin{lemma}\label{lm:dist} Let $t$ be a node of $T$ at level $i$ corresponding to a point $x \in X$, for any leaf $y$ of the subtree rooted at $t$, $d(x,y)\leq  L_i/(1-\epsilon) \leq 2L_i$.
\end{lemma}
 
 For each node $t\in T$, let $\Gamma_t$ be the set of ``adjacency'' orderings of children of $t$. That is, for every two children $u,v$, there exists an ordering $\gamma \in \Gamma_t$ where $u$ and $v$ are adjcent in $\gamma$. By Lemma~\ref{lm:children},  we have:
 
  \begin{equation}\label{eq:adj-ordering-child}
	|\Gamma_t| = O(\epsilon^{-d})
 \end{equation}
 
We then impose an (arbitrary) linear order on $\Gamma_t$; we denote by $\gamma_i$ the $i$-th linear order of $\Gamma_t$. Again, we assume that each node has exactly $q =  O(\epsilon^{-d})$ adjacency ordering (by duplicating if neccessary). We now construct a set of exactly $q$ linear orders $\Sigma$ from $T$ as in Algorithm~\ref{alg:linear-ordering}.


\begin{algorithm}[H]
	\SetAlgoLined
	\DontPrintSemicolon	
	Let $r_T$ be the root of tree $T$;
	
	$\Sigma = \emptyset$;
	
	\ForEach{$ i  \leftarrow 1$ to $q$}
	{ %\eIf{$ f_i = Negated $}
		%{$ N \longleftarrow f_i;$}
		%{$ S \longleftarrow f_i;$}
		$\sigma \leftarrow$ \texttt{Linearize}($r_T,i$);
		
		$\Sigma\leftarrow \Sigma \cup \{\sigma\}$;
	}
	\SetKwFunction{FMain}{Linearize}
	\SetKwProg{Fn}{Function}{:}{}
	\Fn{\FMain{$t,i$}}{
		$ \sigma_t \leftarrow \emptyset$;    
		
		\ForEach{child $ z \in \gamma_i$ of $t$}
		{ $\sigma_z \leftarrow$  \texttt{Linearize}($z,i$);
			
			$\sigma_t \leftarrow\sigma_t \circ \sigma_z$;
		}
		\textbf{return} $ \sigma_t; $ 
	}
	\textbf{End Function}
	\caption{Constructing a linear order}
	\label{alg:linear-ordering}
\end{algorithm}
 
 \begin{lemma}\label{lm:num-ordering}
 	The number of orderings is $O_d(\epsilon^{-d}\log \frac{1}{\epsilon})$.
 \end{lemma}
 \begin{proof}
 	The number is $O(\log \frac{1}{\epsilon})\times p \times q = O_d(\epsilon^{-d}\log\frac{1}{\epsilon})$.
 \end{proof}
 
 It remains to argue that for every pair $(x,y)$, they are properly ordered in some ordering $\sigma$.  Let $\mathcal{H}_k$ be the hierarchy that covers $(x,y)$. Let $i$ be the level of $(x,y)$, i,e, $d(x,y)\in (L_{i/2}, L_i]$.
 

Let $t_x$ and $t_y$ be two ancestors  of $x$ and $y$ in $T$ at level $i-1$. By Lemma~\ref{lm:dist}, $d(x,t_x) \leq 2L_{i-1}$ and $d(y,t_x) \leq 2L_{i-1}$. By definition of $\mathcal{H}_k$ there is a cluster $C$ at level $i$ that contains $B(x,4L_{i-1})$ and $B(y, 4L_{i-1})$. Thus, $t_x$ and $t_y$ are both children of the same node $t$ at level $i$, and hence, there is an ordering  $\gamma_j \in \Gamma_t$ where $t_x$ and $t_y$ are adjacent. Thus, $x$ and $y$ are properly order in the $j$-th ordering of $\Sigma$. 



\end{proof}



\subsection{LSO for Doubling metrics}
{\Huge \color{red} This subsection is some draft of Arnold. Use if needed, or remove.} 

\begin{theorem}
	Consider a metric space $\left(X,d_{X}\right)$ of doubling dimension
	$d$, and parameters $\Delta,\epsilon$. Then $X$ admits $\left(O(\epsilon)^{-d},\epsilon,\Delta\right)$-LSO.
\end{theorem}

\begin{proof}
	We will use the following result from {[}Filtser19{]}:
	\begin{lemma}[\cite{Fil19padded}] 
		Consider a metric space $\left(X,d_{X}\right)$ of
		doubling dimension $d$, and parameters $\Delta$, then for every
		$t=\Omega(1)$, there is a set of $O(2^{\frac{d}{t}}\cdot d\cdot\log t)$
		partitions, such that every pair of points at distance at most $\Delta$
		belongs to some cluster in some partition, and every cluster in every
		partition has diameter at most $O(t)\cdot\Delta$.
	\end{lemma}
	
	Take $t$ to be an obsolute constant, and produce the set of partitions
	from the lemna. For every partition $\mathcal{P}$, we will create
	a set of orderings. Consider a cluster $C\in\mathcal{P}$. Let $N_{C}$
	be a $\frac{\epsilon}{2}\Delta$ net, and create a partition $\mathcal{P}_{C}$
	of $C$ where each vertex goes to the Voronoi cell of the closest
	net point. Note that $|N_{C}|=\left\lceil \frac{O(t)\cdot\Delta}{\frac{\epsilon}{2}\Delta}\right\rceil ^{d}=O(\epsilon)^{-d}$.
	Next we use the following lemma:
	\begin{lemma}
		{[}Alspach08{]} For a set of $n$ elements, there is a collection
		of $\left\lceil \frac{n}{2}\right\rceil $ orderings such that every
		two elements are adjesent is some ordering.
	\end{lemma}
	
	For each partition we create $O(\epsilon)^{-d}$ orderings using the
	lemma above, where in each cluster the points are partitioned arbitrarily.
	In total we obtain a set of $O(\epsilon)^{-d}\cdot O(2^{\frac{d}{t}}\cdot d\cdot\log t)=O(\epsilon)^{-d}$
	orderings. It is strightforward that the theorem holds.
\end{proof}
Next one might wish to generlize this to every distance $\Delta$.
One simple solution will be to take all posible scales:
\begin{corollary}
	Consider a metric space $\left(X,d_{X}\right)$ of doubling dimension
	$d$, and parameter $\epsilon$. Then $X$ admits $\left(O(\epsilon)^{-\left(d+1\right)}\log\Phi,\epsilon\right)$-LSO,
	where $\Phi$ is the aspect ratio.
\end{corollary}

\begin{proof}
	Take the construction above for every $\Delta=(1+\epsilon)^{i}$.
	Then the number of ordering will be $O(\epsilon)^{-d}\log{}_{1+\epsilon}\Phi=O(\epsilon)^{-\left(d+1\right)}\log\Phi$.
\end{proof}
However, it will be nice to get rid of the depandance on $\Phi$. 
\begin{theorem}
	Consider a metric space $\left(X,d_{X}\right)$ of doubling dimension
	$d$, and parameter $\epsilon$. Then $X$ admits $\left(O(\epsilon)^{-\left(d+1\right)}\log\frac{n}{\epsilon},\epsilon\right)$-LSO.
\end{theorem}

\begin{proof}
	Suppose minimal distance is $1$, and maximal distance is $\Phi$.
	For sacle $i\in[0,\log_{1+\epsilon}\Phi]$ let $X_{i}$ be the set
	of points $X$, where every pair at distance at most $O(\frac{\epsilon}{n})$
	is contracted. Set $\ell=\log_{1+\epsilon}\frac{2n}{\epsilon}+O(1)$.
	We will use the same orderings for $\dots,X_{i-2\ell},X_{i-\ell},X_{i},X_{i+\ell},X_{i+2\ell},\dots$.
	This is done as follows: Start with the maximum set. Then for the
	next one, we can simply partition each super node (as all rellevant
	pairs are inside), and so on. One might also observe that the total
	demage from contraction is neglaigble. We conclude that the total
	number of orderings will be $O(\epsilon)^{-d}\ell=O(\epsilon)^{-(d+1)}\log\frac{n}{\epsilon}$.
\end{proof}
Now we can use the construction of oblivious reliable spanners from \cite{BHO19} using orderings. Recall that for the case of $M$ orderings,
they defines $\vartheta'=\frac{\vartheta}{3MN}$ where $N=\log\log n$.
Then for each oredering we construct a spanner with $O(n\frac{1}{\vartheta'}\log\frac{1}{\vartheta'})$
edges. In total, the required number of edges is

\begin{align*}
M\cdot O(n\frac{1}{\vartheta'}\log\frac{1}{\vartheta'}) & =M\cdot O(n\frac{MN}{\vartheta}\log\frac{MN}{\vartheta})\\
& =\frac{n}{\vartheta}\log\log n\cdot O(\epsilon)^{-2(d+1)}\log^{2}\frac{n}{\epsilon}\cdot\log\frac{O(\epsilon)^{-(d+1)}\log\frac{n}{\epsilon}}{\vartheta}\\
& =n\cdot O(\epsilon)^{-2(d+1)}\tilde{O}(\log^{2}\frac{n}{\epsilon})\cdot\frac{1}{\vartheta}\log\frac{1}{\vartheta}
\end{align*}
 
